Incorporating Heterophily into Graph Neural Networks for Graph Classification

Graph Neural Networks (GNNs) often assume strong homophily for graph classification, seldom considering heterophily, which means connected nodes tend to have different class labels and dissimilar features. In real-world scenarios, graphs may have nodes that exhibit both homophily and heterophily. Failing to generalize to this setting makes many GNNs underperform in graph classification. In this paper, we address this limitation by identifying three effective designs and develop a novel GNN architecture called IHGNN (short for Incorporating Heterophily into Graph Neural Networks). These designs include the combination of integration and separation of the ego- and neighbor-embeddings of nodes, adaptive aggregation of node embeddings from different layers, and differentiation between different node embeddings for constructing the graph-level readout function. We empirically validate IHGNN on various graph datasets and demonstrate that it outperforms the state-of-the-art GNNs for graph classification.

==> sec_ethics.tex <==
\section{Ethical Statement}
As many popular GNNs implicitly assume that graphs have nodes of high homophily ratios, the results of such GNNs may be biased, unfair, or erroneous if they are applied to graphs having nodes of low homophily ratios. As can be seen from this paper, atoms (nodes) in molecules tend to connect to atoms from different classes. Without explicitly considering heterophily in the design of GNNs may bring critical problems. Our method IHGNN considers both the homophily and heterophily in the design of $\mbox{COMBINE}^{(k)}(\cdot)$ operator and the graph-level readout function of GNNs, rectifying some possible unethical issues raised by GNNs on heterophilous graphs.
